Modeling and Optimal Operation of Distributed Battery Storage in Low Voltage Grids

Due to high power in-feed from photovoltaics, it can be expected that more battery systems will be installed in the distribution grid in near future to mitigate voltage violations and thermal line and transformer overloading. In this paper, we present a two-stage centralized model predictive control scheme for distributed battery storage that consists of a scheduling entity and a real-time control entity. To guarantee secure grid operation, we solve a robust multi-period optimal power flow (OPF) for the scheduling stage that minimizes battery degradation and maximizes photovoltaic utilization subject to grid constraints. The real-time controller solves a real-time OPF taking into account storage allocation profiles from the scheduler, a detailed battery model, and real-time measurements. To reduce the computational complexity of the controllers, we present a linearized OPF that approximates the nonlinear AC-OPF into a linear programming problem. Through a case study, we show, for two different battery technologies, that we can substantially reduce battery degradation when we incorporate a battery degradation model. A further finding is that we can reduce battery losses by 30% by using the detailed battery model in the real-time control stage.

==> myacronyms.tex <==

\acrodef{etaload}[$\eta_{\mathrm{load}}$] {charge efficiency}
\acrodef{etagen}[$\eta_{\mathrm{gen}}$] {discharge efficiency}
\acrodef{R}[$R$] {internal resistance}
\acrodef{cw}[$c_{\mathrm{w}}$] {charge well factor}
\acrodef{SOC}[SOC]{state of charge}
\acrodef{cr}[$c_{\mathrm{r}}$] {recovery factor}
\acrodef{Q}[$Q_{\mathrm{bat}}$] {charge capacity}
\acrodef{C}[$C_{\mathrm{bat}}$] {energy capacity}
\acrodef{Voc}[$\bar{V}_{\mathrm{oc}}$] {average open circuit potential}
\acrodef{Is}[$I_{\mathrm{s}}$]{side current}
\acrodef{vt}[$V_{\mathrm{t}}$]{terminal voltage}
\acrodef{ibat}[$I_{\mathrm{bat}}$]{battery current}
\acrodef{pbat}[$P_{\mathrm{bat,r}}$]{battery power}
\acrodef{cost}[$c_\mathrm{inv}$]{investment cost}
\acrodef{x}[$x$]{state variable for non-linear and linear battery models. Corresponds to SOC}
\acrodef{x_ex}[$\vec{x}$]{state vector containing $[x_1,x_2]^T$ for the extended non-linear and linear models.}
\acrodef{a}[$a$]{SOC target}
\acrodef{b}[$b$]{cost parameter SOC}
\acrodef{c}[$c$]{cost parameter $u_{\mathrm{gen}}$}
\acrodef{d}[$d$]{cost parameter $u_{\mathrm{load}}$}
\acrodef{e}[$e$]{cost parameter $u_{\mathrm{load}}^2$}
\acrodef{cnet}[$c_{\mathrm{net}}$]{net tariff}
\acrodef{ncell}[$n_{\mathrm{cell}}$]{number of DUALFOIL cells in series}
\acrodef{Acell}[$A_{\mathrm{cell}}$]{cell area}
\acrodef{dclink}[$v_{\mathrm{DC}}$]{DC link voltage}
\acrodef{pthreshold}[$u_{\mathrm{gen,net}}^{\mathrm{max}}$]{peak shave threshold}
\acrodef{horizonT}[$H_{\mathrm{t}}$]{time horizon}
\acrodef{updateT}[$R_{\mathrm{t}}$]{receding horizon window}
\acrodef{sampleTime}[$T_{\mathrm{s}}$]{sample rate}
\acrodef{rsa}[$r_{\mathrm{sa}}$]{side reaction rate constant anode}
\acrodef{rsc}[$r_{\mathrm{sc}}$]{side reaction rate constant cathode}
\acrodef{unet}[$u_{\mathrm{gen}}^{\mathrm{net}}$]{}
\acrodef{unetmax}[$u_{\mathrm{gen,max}}^{\mathrm{net}}$]{}
\acrodef{ubatgen}[$u_{\mathrm{gen}}^{\mathrm{bat}}$]{}
\acrodef{ubatload}[$u_{\mathrm{load}}^{\mathrm{bat}}$]{}
\acrodef{uloadG2}[$P_{\mathrm{load}}^{\mathrm{G2}}$]{G2 standard industrial load profile}
\acrodef{Qs}[$Q_{\mathrm{s}}$]{lost charge}

\acrodef{ID}[ID]{Identification}
\acrodef{NLS}[NLS]{Nonlinear Least Squares}
\acrodef{LS}[LS]{Least Squares}
\acrodef{MPC}[MPC]{Model Predictive Control}
\acrodef{QP}[QP]{Quadratic Programming}
\acrodef{MSE}[MSE]{Mean Squared Error}
\acrodef{RMSE}[RMSE]{Root Mean Squared Error}
\acrodef{NRMSE}[NRMSE]{Normalized Root Mean Squared Error}


==> optimalControl.tex <==

\section{Optimal Battery Operation}
\label{sec:control}
\subsection{Control Structure}
As shown in Fig.~\ref{fig:scheduler} our proposed control scheme consists of two control entities working at different time scales. We do not allow for PV curtailment and so the scheduler has to calculate future storage allocation bounds in terms of energy $\vec{e}_\mathrm{min},\vec{e}_\mathrm{max}$ and aggregated power $p_\mathrm{bat}^{\mathrm{agg}}$ that are feasible under the worst case \ac{PV} forecast scenarios. The \ac{RT} controller tries to control the storage units within these bounds, while minimizing network and storage losses and taking into account \ac{RT} measurements of the net load.          
\begin{figure}[!t]
	\centering
	\def\svgwidth{\columnwidth}
	\input{scheduler.pdf_tex}
	\caption{Centralized control scheme consisting of a scheduler and an \ac{RT} controller. The scheduler uses robust \ac{MPC}. The \ac{RT} controller solves a \ac{RT}-\ac{OPF} using the storage allocation from the scheduler and \ac{RT} measurements.}
	\label{fig:scheduler}
\end{figure}


\subsection{Scheduler}
\label{sec:scheduler}
We solve a robust multi-period \ac{OPF} subject to the worst case PV predictions. Since we solve the multi-period problems in a receding horizon fashion every hour with updated energy levels, the scheduler acts as a robust \ac{MPC}. 
\subsubsection{Incorporation of Distributed Storage}
Due to its high sample time $T_1=1$ hour, the scheduler cannot capture the detailed battery dynamics so we use the linear basic model~\eqref{eq:linearbasic}. The discrete version of \eqref{eq:linearbasic} for $n_s$ battery systems is    
\begin{equation}
\resizebox{1\hsize}{!}{$\vec{e}(k+1)  = \vec{I}^{n_s}\vec{e}(k) + 
\underbrace{T_1 \left[ \mathrm{diag}\{-\vec{\eta}_\mathrm{dis}^{-1}\} \ \mathrm{diag}\{-\vec{\eta}_\mathrm{ch}\} \right]}_{\vec{B}} \underbrace{\left[\begin{array}{l} \vec{p}_\mathrm{gen}^\mathrm{s,dis} \\ \vec{p}_\mathrm{gen}^\mathrm{s,ch} \end{array}\right]}_{\vec{p}_\mathrm{gen}^\mathrm{s}}$} ,						
\end{equation}
\noindent where $\vec{p}_\mathrm{gen}^\mathrm{s,dis} \geq \vec{0} \in \mathbb{R}^{n_s \times 1}$, $\vec{p}_\mathrm{gen}^\mathrm{s,ch} < \vec{0} \in \mathbb{R}^{n_s \times 1}$, 
%are the discharging and charging powers  -- JM removed because previously defined
$\vec{\eta}_\mathrm{dis},\vec{\eta}_\mathrm{ch} \in \mathbb{R}^{n_s \times 1}$ are the total discharging and charging efficiencies of the storage units, and $\vec{I}^{n_s}$ denotes the identity matrix of dimension $n_s$.
The complete SoE evolution $\vec{E} = [\vec{e}(1),...,\vec{e}(N-1)]^T$ for a time horizon of length $N$ is
\begin{equation}
\vec{E} =  \underbrace{\left[ \begin{array}{c} \vec{I}^{n_s} \\ \vdots \\ \vec{I}^{n_s}\end{array} \right]}_{\vec{S}_x}\vec{e}(0) + \underbrace{\left[\begin{array}{ccc}  \vec{B}  &  & \vec{0} \\ \vdots &\ddots \\ \vec{B} & \cdots & \vec{B} \end{array}\right]}_{\vec{S}_u}\underbrace{\left[\begin{array}{l} \vec{p}_\mathrm{gen}^\mathrm{s}(0) \\ \vdots \\  \vec{p}_\mathrm{gen}^\mathrm{s}(N-1) \end{array} \right]}_{\vec{U}} \quad, \label{eq:evo}
\end{equation}
\noindent where $\vec{e}(0)$ is the initial SoE vector.

\subsubsection{Incorporation of Battery Degradation}
In Section~\ref{sec:convexhull} we calculated the \ac{PWA} convex hull \eqref{eq:hull} of the degradation map. To incorporate degradation into the planning problem, we define helper decision variables $\vec{Z} = [\vec{z}(0),\hdots,\vec{z}(N-1) \in \mathbb{R}^{n_s\times 1}]^T$ and include the epigraphs of \eqref{eq:hull} as constraints in our problem. %By substituting the $SoE$ vector $\vec{E}$ with the control variable $\vec{U}$ in \eqref{eq:evo}, we express the epigraphs of \eqref{eq:hull} with respect to $\vec{U}$ and obtain   
Specifically, we substitute $\vec{E}$ from \eqref{eq:evo} into an extended version of \eqref{eq:hull} that includes $n_s$ battery systems with energy capacities $\vec{c}_\mathrm{E} \in \mathbb{R}^{n_s \times 1}$ and obtain a degradation equation in terms of the control variable $\vec{U}$ as follows:
\begin{equation}
\left(\vec{A}_1+\vec{A}_2\vec{S}_u\right) \vec{U} + \vec{A}_z\vec{Z} \leq -\vec{A}_2\vec{S}_x\vec{e}_0-\vec{A}_3\vec{c}_\mathrm{E} \label{eq:batdeg}\quad,
\end{equation}
where $\vec{A}_1 = [\vec{I}^{N n_s}\otimes \vec{a}_1 ][\vec{I}^{N} \otimes [\vec{I}^{Nn_s} \vec{I}^{Nn_s}]]$, $\vec{A}_2 = [\vec{I}^{N n_s }\otimes \vec{a}_2]$, $\vec{A}_3 = \vec{I}^{N} \otimes [\vec{I}^{n_s} \otimes \vec{a}_3 ]$, and $\vec{A}_z = [\vec{I}^{N n_s}\otimes -\vec{1}^{n_{\mathrm{p}}\times 1} ]$. The operator $\otimes$ denotes the Kronecker product. 

\subsubsection{Robust Scheduling}
To solve a multi-period \ac{OPF} we first incorporate a temporally-coupled sequence of single period OPF problems \eqref{eq:FBOPF}. We extend the decision vector to $\vec{X} = [\vec{x}_0,\cdots,\vec{x}_{N-1}]^T$, where $\vec{p}_{\mathrm{gen},k} = [{p}_{\mathrm{net}}(k) \ \vec{p}_{\mathrm{gen}}^{\mathrm{s}}(k) ]^T \in \vec{x}_k$ and ${p}_{\mathrm{net}}(k)$ (i.e., the net power into or out of the LAC) is treated as a slack generator.
%and the vector $\vec{p}_{\mathrm{gen},i}^{\mathrm{s}} \in \mathbb{R}^{2n_s\times 1}$ reflects the charging and discharging battery powers. -- JM removing because already defined
Since we do not allow for PV curtailment, we set 
\begin{equation}
\vec{p}_{\mathrm{d},k} = -\vec{C}_\mathrm{pv} (\hat{\vec{p}}_{\mathrm{gen},k}^{\mathrm{pv}}+\vec{w}_k3\vec{\sigma}_{\mathrm{pv},k}^T) + \hat{\vec{p}}_{\mathrm{ld},k}\quad,
\end{equation} 
\noindent where the PV and load forecasts are denoted by $\hat{\vec{p}}_{\mathrm{gen},k}^{\mathrm{pv}}$ and $\hat{\vec{p}}_{\mathrm{ld},k}$, and $\vec{C}_\mathrm{pv} \in \mathbb{R}^{n\times n_{\mathrm{pv}}}$ maps the $n_{\mathrm{pv}}$ \ac{PV} units to the buses. The standard deviation {$\vec{\sigma}_{\mathrm{pv},k}$ of the PV forecast error could be determined by using the results from \cite{Bacher}. We define $\vec{W} = [\vec{w}_0,\hdots,\vec{w}_{N-1}]^T$, which is a box-constrained uncertainty set where $\vec{-1}\leq \vec{W} \leq \vec{1}$. Note that we do not consider load forecast uncertainty, since absolute load forecast errors are generally much smaller than absolute PV forecast errors for a grid with high PV penetration. The scheduling problem is 
\begin{equation}
	\begin{array}{llll}
		\multicolumn{4}{l} {\displaystyle\min_{\vec{X},\vec{Z}} \ T_1 \left(\sum\limits_{k=0}^{N-1} \ {c}_{\mathrm{n}} {p}_{\mathrm{net}}(k)  + {c}_{\mathrm{d}} \vec{1}^T\vec{z}(k) \right)}\\
		 \text{s.t.} & \text{(a)} & \multicolumn{2}{l}{ -\vec{S}_x\vec{e}(0) \leq \vec{S}_u {\vec{U}} \leq \vec{c}_{\mathrm{E}} - \vec{S}_x\vec{e}(0) }\\
		  & & \multicolumn{2}{l}{\forall \vec{x}_k: \displaystyle\max_{-\vec{1} \leq \vec{W} \leq \vec{1}} \text{(\ref{eq:FBOPF}{a-c,e})} ,\text{(\ref{eq:FBOPF}{d,g-l}),{\eqref{eq:batdeg}}} \ ,}  
			\end{array}
	\label{eq:robustProb} 
\end{equation}
\noindent where $c_\mathrm{n}$ and $c_\mathrm{d}$ are cost parameters for the net power and the battery degradation. With this formulation, the PV infeed will be maximized since the optimizer minimizes $p_\mathrm{net}$. The constraint set (\ref{eq:robustProb}a) operates the storage devices at their minimum and maximum bounds.
To retrieve the robust counterpart of \eqref{eq:robustProb}, we eliminate $\vec{w}_k$ and use $|\vec{\sigma}_{\mathrm{pv},k}|$ within each constraint \cite{bental}, since \vec{X} does not multiply the random variable \cite{Lofberg2012}.
\subsubsection{Determination of Robust Storage Level Bounds}
To link the planning domain with the \ac{RT} domain, the scheduler sends robust allocation bounds for the \ac{RT} controller
\begin{eqnarray}
\vec{e}_\mathrm{min}& = &\min(\vec{e}(0),\vec{e}(1)) \\
\vec{e}_\mathrm{max}& = &\max(\vec{e}(0),\vec{e}(1)) \quad ,
\end{eqnarray}
\noindent where we evaluate $\vec{e}(1)$ with \eqref{eq:evo}. The scheduler also sends the aggregated battery setpoint $p_\mathrm{bat}^{\mathrm{agg}}$ to give the \ac{RT} controller the ability to operate the batteries at their individual optimal operation points
\begin{equation}
p_\mathrm{bat}^{\mathrm{agg}}  =  \vec{1}^T \vec{p}_\mathrm{gen}^{*\mathrm{s}}(1) \quad,
\end{equation}
where $\vec{p}_\mathrm{gen}^{*\mathrm{s}}(1)$ is a portion of the optimal decision vector of the robust problem \eqref{eq:robustProb}. 

\begin{figure}[!t]
	\centering
	\def\svgwidth{\columnwidth}
	\input{controlArchi.pdf_tex}
	\caption{Block diagram of the \ac{RT} controller.}
	\label{fig:rtControl}
\end{figure}  

\subsection{Real-Time Control}
\label{sec:RTcontrol}
As depicted in Fig.~\ref{fig:rtControl}, the \ac{RT} controller receives the storage allocation bounds and aggregated battery power setpoint. Using \ac{RT} measurements of the PV injections $\vec{p}_{\mathrm{gen}}^{\mathrm{pv}},\vec{q}_{\mathrm{gen}}^{\mathrm{pv}}$ and loads $\vec{p}_\mathrm{ld},\vec{q}_\mathrm{ld}$ to compute $\vec{p}_\mathrm{d},\vec{q}_\mathrm{d}$, it sets the reactive and active battery powers $\vec{p}_\mathrm{gen}^\mathrm{s},\vec{q}_\mathrm{gen}^\mathrm{s}$ by solving an RT-OPF. In particular, we solve an MPC problem for one step incorporating the linear extended battery model \eqref{eq:extend}, allowing us to estimate the power available from each individual battery system and utilize its full capacity potential. The decision vector is $\vec{u}_0 = [\vec{p}_\mathrm{gen}^\mathrm{s} \ \vec{q}_\mathrm{gen}^\mathrm{s} \ \vec{\lambda} \ \vec{p}_{\mathrm{bat}}^{\mathrm{loss}} \ \ y_\mathrm{set}^{\mathrm{agg}} \ \vec{x}_\mathrm{set}]^T$, where $\vec{\lambda}$ and $\vec{p}_{\mathrm{bat}}^{\mathrm{loss}}$ are helper variables to incorporate battery losses into the problem and $ y_\mathrm{set}^{\mathrm{agg}}$ and $\vec{x}_\mathrm{set}$ are helper variables to penalize deviations from the storage allocation bounds. The RT-OPF problem is
\begin{equation}
\begin{array}{lllll}
\displaystyle \min_{\vec{u}_0} 
&  \multicolumn{4}{l}{\underbrace{\vec{1}^T\vec{p}_{\mathrm{gen}}}_{\text{network losses}} + \underbrace{\vec{1}^T\vec{p}_{\mathrm{bat}}^{\mathrm{loss}} }_{\text{battery losses}} + \underbrace{ y_\mathrm{set}^{\mathrm{agg}} + \vec{1}^T \vec{x}_\mathrm{set}}_{\text{deviations from setpoint regions}}}\\
\hspace{0.2cm}\text{s.t.}   
& \multicolumn{4}{l}{(\ref{eq:FBOPF}\mathrm{a})-(\ref{eq:FBOPF}\mathrm{l})} \\
& \text{(a)} & \vec{X}_1& = & \vec{\Phi} \vec{X}_0 + \vec{H} \vec{p}_\mathrm{gen}^\mathrm{s} \\
& \text{(b)} & \vec{0} &\leq  &\vec{X}_1 \leq \vec{1}^{n_s \times 1} \otimes \left[ \begin{array}{c}
c_\mathrm{w} \\ 1-c_\mathrm{w} \end{array} \right] \\
& \text{(c)} & \multicolumn{3}{l}{-\operatorname{diag}\{\vec{m} \}\vec{C}\vec{X}_1 - \vec{I}^{n_s}\vec{x}_\mathrm{set} \leq  -\vec{e}_\mathrm{min}m}  \\
& \text{(d)} & \multicolumn{3}{l}{\operatorname{diag}\{\vec{m} \}\vec{C}\vec{X}_1 - \vec{I}^{n_s}\vec{x}_\mathrm{set} \leq  \vec{e}_\mathrm{max}m}  \\
& \text{(e)} & \multicolumn{3}{l}{ \vec{I}^{n_s}\vec{x}_\mathrm{set} \leq  \vec{0}} \\
& \text{(f)} & \multicolumn{3}{l}{ -m \vec{1}^T \vec{p}_{\mathrm{gen}}^{\mathrm{s}} - y_\mathrm{set}^{\mathrm{agg}}   \leq  -m {p}_{\mathrm{bat}}^{\mathrm{agg}}}   \\
& \text{(g)} & \multicolumn{3}{l}{  - y_\mathrm{set}^{\mathrm{agg}}   \leq  0 }  \\
& \text{(h)} & \multicolumn{3}{l}{\vec{p}_\mathrm{d} = -\vec{C}_\mathrm{pv} {\vec{p}}_{\mathrm{gen}}^{\mathrm{pv}} + {\vec{p}}_\mathrm{ld} } \\
& \text{(i)} & \multicolumn{3}{l}{\vec{q}_\mathrm{d} = -\vec{C}_\mathrm{pv} {\vec{q}}_{\mathrm{gen}}^{\mathrm{pv}} + {\vec{q}}_\mathrm{ld} } \\
& \text{(j)} & \multicolumn{3}{l}{-\vec{I}^{n_s} \vec{p}_\mathrm{gen}^\mathrm{s} + \left[\vec{I}^{n_s} \otimes \vec{p}_\mathrm{gen}^{\mathrm{s},P}\right]  \vec{\lambda} = \vec{0}  } \\
& \text{(k)} & \multicolumn{3}{l}{-\vec{I}^{n_s}  \vec{p}_{\mathrm{bat}}^{\mathrm{loss}} + \left[\vec{I}^{n_s} \otimes f(\vec{p}_\mathrm{gen}^{\mathrm{s},P})\right]  \vec{\lambda} = \vec{0}  } \\
& \text{(l)} & \multicolumn{3}{l}{\left[\vec{I}^{n_s} \otimes \vec{1}^{1\times n_s}\right]  \vec{\lambda} = \vec{1}  }\\
& \text{(m)} & \multicolumn{3}{l}{\vec{\lambda} = [\vec{\lambda}_1,\hdots,\vec{\lambda}_{n_s}]^T \ \forall \vec{\lambda}_i : \text{SOS2} \quad, }
\end{array}
\label{eq:mpc}
\end{equation}
\noindent where (\ref{eq:mpc}a) is the discrete version of \eqref{eq:extend} for multiple battery systems. Specifically, $\vec{X}_0$ is the initial battery system state and $\vec{X}_1$ is the state after one time step; \vec{\Phi} is the battery system dynamics matrix, $\vec{H}$ is the RT control input matrix, and $\vec{C}$ maps the internal states of each battery system to the SoE. Constraint (\ref{eq:mpc}b) avoids overspill of the battery capacity wells. Constraints (\ref{eq:mpc}c-e) define two regions and enable us to penalize deviations outside of the storage allocation bounds $\vec{e}_\mathrm{min},\vec{e}_\mathrm{max}$  with the penalty factor $m$, where $\operatorname{diag}\{\vec{m}\}$ is a square matrix with $m$ on the diagonal. We only penalize the aggregated power setpoint in the discharging direction with (\ref{eq:mpc}f,g), since overcharging can be dealt with in \ac{RT} as it will not result in line limit violations. This yields lower storage utilization and thus results in lower battery degradation.
Constraints (\ref{eq:mpc}h,i) incorporate the \ac{RT} measurements and (\ref{eq:mpc}j-m) represent nonconvex piecewise linear functions of the battery losses using an efficient \ac{SOS} formulation \cite{sos2}. In particular, we discretize \eqref{pbatloss} with $P$ supporting points $\vec{p}_\mathrm{gen}^{\mathrm{s},P}$ and evaluate \eqref{pbatloss} for each point and for each battery system. The sum of the elements in the set $\vec{\lambda}_i$ has to be equal to 1, which is enforced in (\ref{eq:mpc}l), and at most two elements in the set have to be consecutively non-zero (\ref{eq:mpc}m). This is referred to as an \ac{SOS}2 set. Constraint (\ref{eq:mpc}m) makes the problem a Mixed Integer Linear Programming (MILP) problem.  

We also implemented an observer to estimate the internal states $\vec{x}_\mathrm{E}$ of each individual battery system, since battery management systems typically provide only the SoE. Since the system \eqref{eq:extend} is detectable, \cite{observer} we can design following Luenberger observer
\begin{equation}
\dot{\hat{\vec{x}}}_\mathrm{E} = (\vec{A} -\vec{l} [1 \ 1])\hat{{\vec{x}}}_\mathrm{E} + \left[\begin{array}{cc}
\begin{array}[h]{c}
1  \\
0 \\
\end{array} & \vec{l}\end{array}\right] 
\left[
\begin{array}[h]{c}
P_\mathrm{bat}  \\
E \\
\end{array}\right] \quad,
\end{equation}
\noindent where $\vec{l} \in \mathbb{R}^{2\times 1}$ is chosen such that $(\vec{A}-\vec{l}[1 \ 1])$ is stable. 


%\noindent where $P_{\mathrm{bat}} = \sum\limits_{k=1}^{l} \lambda_k P_{\mathrm{bat}}^k$ and $\sum\limits_{k=1}^{l}\lambda_k = 1$ define $l$ piece-wise linear segments and the $\lambda_k$ represent a \ac{SOS} of type 2 \cite{cplex}.


